EL PASSO: Privacy-preserving, Asynchronous Single Sign-On

We introduce EL PASSO, a privacy-preserving, asynchronous Single Sign-On (SSO) system. It enables personal authentication while protecting users' privacy against both identity providers and relying parties, and allows selective attribute disclosure. EL PASSO is based on anonymous credentials, yet it supports users' accountability. Selected authorities may recover the identity of allegedly misbehaving users, and users can prove properties about their identity without revealing it in the clear. EL PASSO does not require specific secure hardware or a third party (other than existing participants in SSO). The generation and use of authentication credentials are asynchronous, allowing users to sign on when identity providers are temporarily unavailable. We evaluate EL PASSO in a distributed environment and prove its low computational cost, yielding faster sign-on operations than OIDC from a regular laptop, one-second user-perceived latency from a low-power device, and scaling to more than 50 sign-on operations per second at a relying party using a single 4-core server in the cloud.

==> Makefile <==
PRJ = main

.PHONY: all view clean

all : ${PRJ}.pdf

${PRJ}.pdf : *.tex *.bib
	pdflatex ${PRJ}
	bibtex ${PRJ}.aux
	pdflatex ${PRJ}
	pdflatex ${PRJ}
	# pdflatex ${EXTRA} ${PRJ} && \
	# 	(ls ${PRJ}.aux | xargs -n 1 bibtex) && \
	# 	pdflatex ${EXTRA} ${PRJ} && pdflatex ${EXTRA} ${PRJ}

tarball :
	rm -f el-passo.tar.gz
	tar -cvzf el-passo.tar.gz *.tex images/*.pdf plots/*.png *.sty *.bbl

view : ${PRJ}.pdf
	open ${PRJ}.pdf &

clean:
	rm -Rf latex.out
	rm -f *.toc *.aux *.bbl *.blg *.log *~* *.bak *.out *synctex.gz *.ent *.dvi *.fls *.fdb* ${PRJ}.pdf


==> sections/background.tex <==
%!TEX root = ../usenix/main-usenix.tex
%=========================================================

\vspace{-2mm}
\section{Background}
\label{sec:background}

%While OpenID Connect (OIDC) adheres to some of the design goals listed in Table~\ref{tab:sso_properties}, we identify the design choices of OIDC that are inconsistent with other key target properties\footnote{We also analyze alternative designs and research proposals in Section~\ref{sec:related}, and find no existing system that provides all the identified properties in Table~\ref{tab:sso_properties}.}.
%In the following, we analyze OIDC and present a comparison, illustrated in \Cref{fig:introduction_schema}.

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[scale=0.45]{img/sso}
% 	% \vspace{-10pt}
% 	\caption{A simplified flow of the OIDC protocol.}
% 	\label{fig:sso}
% 	% \vspace{-10pt}
% \end{figure}
\mk{We might want to reduce the description even further and include it in the introduction} \er{this section should go away altogether, so I am keeping it as dead code now. Only the part about web assembly needs to be moved on to the implementation discussion later in the paper.}
\para{Message flow in OIDC} %OIDC is built on top of OAuth - an access delegation protocol, commonly used as a means for users to grant RPs access to information stored at an IdP~\cite{hardt2012oauth}.
%OAuth requires users to give their consent for data sharing once.
%Consequent data transfers happen between the RP and the IdP without user interaction.
%Such an approach allows an RP to access user data even when a user is offline.
OIDC is built on top of OAuth~\cite{hardt2012oauth} - an access delegation protocol, and inherits its tightly \emph{coupled} message flow.
Initially, an RP must \emph{register} with each IdP it wants to support.
The RP receives a secret that will be used later to retrieve user information\footnote{OIDC specification also includes a discovery module allowing RPs to work with IdPs they did not register with beforehand and perform the registration process ``on the fly''. However, this variant is not widely deployed.}.
%Figure~\ref{fig:sso} details the OIDC protocol.
When a user wants to sign on with a website held by an RP, they select one of the IdPs that are supported by that RP.
The RP redirects the user to the chosen IdP including a list of requested attributes (\eg email address, phone number).
The user must then give their consent to share the requested information.
If the access is granted, the IdP responds to the RP with an ID token containing the signed user's identity (if using the ``implicit flow'') or returns an access code allowing RPs to fetch the ID token (when using the ``code flow'').
The code flow requires the RP to use its secret obtained upon registration.
It is suggested as the more secure way of fetching user information, as it does not expose the token to the user's web browser and potentially malicious add-ons.%\footnote{There exists a third ``hybrid'' flow that we omit in this discussion as it does not influence the properties of the protocol.}.
% \zz{According to review A: I suggest we move footnote to be after code flow.} \er{ignored}
%\mk{I'd remove the paragraph below. We already talk about problems of OIDC in the intro}
%Due to this coupling, the design of OIDC is intrinsically unable to provide \emph{user tracking protection}.
%The property of \emph{selective disclosure} is dependent on the goodwill of the IdP, and the lack of \emph{inter-RP unlinkability} makes it possible for an adversary controlling multiple RPs to collect more information than allowed by the user.
%The synchrony in the generation of the authentication token by the IdP and its use with the RP, also prevents OIDC from providing \emph{asynchronous authentication}, requiring the IdP to be always available for users to sign on RPs.


\para{WebAssembly}
WebAssembly (Wasm) is an open standard that defines a portable binary-code format for executable programs, and a corresponding textual assembly language, as well as interfaces for facilitating interactions between such programs and their host environment. WebAssembly code can be run natively in all the major web browsers. Various compilers allow transforming high-level language source code (\ie C++, RUST) into a binary file which runs in the same sandbox as regular JavaScript code.

